Centaurus A: constraints on the nature of the giant lobe filaments from XMM-Newton observations

We report on deep XMM-Newton observations of the vertex filament in the southern giant lobe of the Fanaroff-Riley class I radio galaxy Centaurus A. We find no X-ray excess from the filament region and place a 3 sigma upper limit on the 1 keV flux density of the filament of 9.6 nJy. This directly constrains the electron density and magnetic field strength in the filament. For the first time in an individual filament, we show that so long as the particle index >=2, the excess in synchrotron emissivity cannot be produced purely by excess electrons: the filament magnetic field strength must be higher than in the giant lobes as a whole, and close to or above the equipartition value for the filament. The filaments are not significantly overpressured with respect to the surrounding lobe with a pressure provided by relativistic electrons.

==> journals.tex <==
\bibpunct{(}{)}{;}{a}{}{,}
\def\aap{A\&A}                % Astronomy and Astrophysics
\def\aapr{A\&A~Rev.}          % Astronomy and Astrophysics Reviews
\def\aaps{A\&AS}              % Astronomy and Astrophysics, Supplement
\def\aj{AJ}                   % Astronomical Journal
\def\ajph{Australian J.~Phys.}% Australian Journal of Physics
\def\alet{Astro.~Lett.}       % Astronomical Letters
\def\ao{Applied Optics}       % Applied Optics
\def\apj{ApJ}                 % Astrophysical Journal
\def\apjl{ApJ}                % Astrophysical Journal, Letters
\def\apjs{ApJS}              % Astrophysical Journal, Supplement
\def\apss{Ap\&SS}             % Astrophysics and Space Science
\def\araa{ARA\&A}             % Annual Review of Astronomy and Astrophysics
\def\asr{Av.~Space Res.}     % Advances in Space Research
\def\azh{AZh}                 % Astronomiceskij Zhurnal
\def\baas{BAAS}               % Bulletin of the American Astronomical Society
\def\cpc{Comput.~Phys.~Commun.} % Computer Physics Communications
\def\gca{Geochim.~Cosmochim.~Acta} % Cheochimica et Cosmochimica Acta
\def\iaucirc{IAU Circ.}       % International Astronomical Union, Circular
\def\ibvs{IBVS}               % International Bulletin of Variable Stars
\def\icarus{Icarus}           % Icarus
\def\jcomph{J.~Comput.~Phys.} % Journal of Computational Physics
\def\jcp{J.~Chem.~Phys.}      % Journal of Chemical Physics
\def\jgr{J.~Geophys.~R.}      % Journal of Geophysical Research
\def\jrasc{JRASC}             % Journal of the RAS of Canada
\def\met{Meteoritics}         % Meteoritics
\def\mmras{MmRAS}             % Memoirs of the Royal Astronomical Society
\def\mnras{MNRAS}             % Monthly Notices of the RAS
\def\mps{Meteoritics and Planetary Science} % Meteoritics and Planetary Science
\def\nast{New Astron.}        % New Astronomy
\def\nat{Nature}              % Nature
\def\pasj{PASJ}               % Publ. of the Astronomical Society of Japan
\def\pasp{PASP}               % Publ. of the Astron. Society of the Pacific
\def\phr{Phys.~Rev.}          % Physical Review
\def\pdra{Phys.~Rev.~A}       % Physical Review A
\def\prb{Phys.~Rev.~B}       % Physical Review B
\def\prc{Phys.~Rev.~C}       % Physical Review C
\def\prd{Phys.~Rev.~D}       % Physical Review D
\def\phrep{Phys.~Rep.}        % Physics Reports
\def\phss{Phys.~Stat.~Sol.}        %
\def\procspie{Proc.~SPIE}     % Proceedings of the SPIE
\def\planss{Planet.~Space Sci.}  % Planetary & Space Sciences
\def\qjras{QJRAS}             % Quarterly Journal of the RAS
\def\rpph{Rep.~Prog.~Phys.}   % Reports on Progress in Physics
\def\rgsp{Rev.~Geophys.~Space Phys.~} % Reviews on Geophysics and Space Physics
\def\sal{Soviet Astron.~Lett.}% Soviet Astronomy Letters
\def\sci{Science}             % Science
\def\solph{Sol.~Phys.}        % Solar Physics
\def\ssr{Space Sci.~Rev.}     % Space Science Reviews
\def\zap{Z.~Astrophys.}       % Zeitschrift fuer Astrophysik

